Dimension-Free Approximate Tensorization of Quantum Hypercontractivity for Qudit Depolarizing Semigroups

We prove approximate tensorization for hypercontractivity and logarithmic-Sobolev constants for a class of primitive reversible quantum Markov semigroups satisfying the positive off-diagonal scaling (PODS) condition. This class includes qubit examples and generalized depolarizing semigroups with respect to full-rank states in arbitrary finite dimensions. For any such semigroup $(\Phi_t)_{t\ge 0}$ and every tensor power $n$, we show that the log-Sobolev constant of the product semigroup $\Phi_t^{\otimes n}$ is at least $2/(3\ln 2)\approx 0.96$ times the log-Sobolev constant of the single-site semigroup $\Phi_t$, independently of $n$ and the local dimension $d$. The proof first establishes an exact tensorization of the $(q,2)$-hypercontractive inequality for integer $q$, in particular $q=3$, and then extends the estimate to all real $q>2$ by complex interpolation; the standard implication from hypercontractivity to logarithmic-Sobolev inequalities yields the stated almost tensorization result. In the qubit case, we further prove exact tensorization for primitive reversible PODS semigroups and obtain sharp $(q,2)$-hypercontractivity estimates for generalized qubit depolarizing channels.

==> preamble.tex <==
\usepackage{hyperref}
\newif\ifTITsubmission
\makeatletter
\@ifclassloaded{IEEEtran}{\TITsubmissiontrue}{\TITsubmissionfalse}
\makeatother

\ifTITsubmission\else
\usepackage{fullpage}
\fi
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{breqn}
\usepackage{amsthm}
\usepackage{dsfont}
\ifTITsubmission\else
\usepackage{libertine}
\fi
\usepackage[capitalise]{cleveref}
\usepackage{thmtools}
\usepackage{mathtools}
\usepackage{booktabs}
\usepackage{array}
\usepackage{tikz}
\usetikzlibrary{positioning,arrows.meta,calc}

\ifTITsubmission\else
\makeatletter
\renewcommand{\section}{\@startsection {section}{1}{\z@}
             {-3.5ex \@plus -1ex \@minus -.2ex}
             {2.3ex \@plus .2ex}
             {\normalfont\Large\scshape\bfseries}}
\renewcommand{\subsection}{\@startsection{subsection}{2}{\z@}
             {-3.25ex\@plus -1ex \@minus -.2ex}
             {1.5ex \@plus .2ex}
             {\normalfont\large\scshape\bfseries}}
\renewcommand{\subsubsection}{\@startsection{subsubsection}{2}{\z@}
             {-3.25ex\@plus -1ex \@minus -.2ex}
             {1.5ex \@plus .2ex}
             {\normalfont\normalsize\scshape\bfseries}}
\makeatother
\fi

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]

\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{prop}[theorem]{Proposition}
\newtheorem{cor}[theorem]{Corollary}
\newtheorem*{maintheorem}{\Cref{thm:main}}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{example}[theorem]{Example}

\makeatletter
\renewcommand*{\theHtheorem}{\theHsection.\arabic{theorem}}
\let\theHlemma\theHtheorem
\let\theHprop\theHtheorem
\let\theHcor\theHtheorem
\let\theHdefinition\theHtheorem
\let\theHclaim\theHtheorem
\let\theHproblem\theHtheorem
\let\theHremark\theHtheorem
\let\theHfact\theHtheorem
\let\theHexample\theHtheorem
\makeatother

